Supersymmetric Yang-Mills theory: a step towards the continuum

The spectrum of supersymmetric Yang-Mills theory presented so far shows an unexpected gap between the bosonic and fermionic masses. This finding was in contradiction with the basic requirements of supersymmetry. In this work we will present new results indicating that the mass gap is reduced at a smaller lattice spacing. Hence lattice artifacts are the most likely explanation for it. These new results have been obtained at a larger beta value and on a larger lattice.

==> PaxHeader/pos_lattice2011.tex <==
16 uid=10014613
30 mtime=1321001939.095631072
30 ctime=1321002015.977747644
20 atime=1321000890
17 SCHILY.dev=25
23 SCHILY.ino=19851974
18 SCHILY.nlink=1

